MultiBiSage: A Web-Scale Recommendation System Using Multiple Bipartite Graphs at Pinterest

Graph Convolutional Networks (GCN) can efficiently integrate graph structure and node features to learn high-quality node embeddings. These embeddings can then be used for several tasks such as recommendation and search. At Pinterest, we have developed and deployed PinSage, a data-efficient GCN that learns pin embeddings from the Pin-Board graph. The Pin-Board graph contains pin and board entities and the graph captures the pin belongs to a board interaction. However, there exist several entities at Pinterest such as users, idea pins, creators, and there exist heterogeneous interactions among these entities such as add-to-cart, follow, long-click. In this work, we show that training deep learning models on graphs that captures these diverse interactions would result in learning higher-quality pin embeddings than training PinSage on only the Pin-Board graph. To that end, we model the diverse entities and their diverse interactions through multiple bipartite graphs and propose a novel data-efficient MultiBiSage model. MultiBiSage can capture the graph structure of multiple bipartite graphs to learn high-quality pin embeddings. We take this pragmatic approach as it allows us to utilize the existing infrastructure developed at Pinterest -- such as Pixie system that can perform optimized random-walks on billion node graphs, along with existing training and deployment workflows. We train MultiBiSage on six bipartite graphs including our Pin-Board graph. Our offline metrics show that MultiBiSage significantly outperforms the deployed latest version of PinSage on multiple user engagement metrics.

==> dump.tex <==
 We select the neighbors with node type equal to pin. The rationale for not selecting user or board neighbors is because user and board embeddings are learnt to pin embeddings. Our goal is to learn pin-embeddings and including user/board embeddings create cyclic dependency which would prevent us to ever deprecating models that learn user and board embeddings. 
 
 
 %     \multirow{2}{*}{Organic Surface} & Add-to-cart	&	0.907	 (+1.57	\%) &	0.900	 (+0.78	\%) &	0.902	 (+1.01	\%) &	0.901	 (+0.90	\%) &	0.899	 (+0.67	\%) &	0.900	 (+0.78	\%)	\\
% & Checkout   	&	0.907	 (+1.57	\%) &	0.898	 (+0.56	\%) &	0.900	 (+0.78	\%) &	0.900	 (+0.78	\%) &	0.901	 (+0.90	\%) &	0.902	 (+1.01	\%)	\\
% \midrule
% Ads Surface & Click-through rate	&	0.684	 (+5.07	\%) &	0.670	 (+2.92	\%) &	0.676	 (+3.84	\%) &	0.669	 (+2.76	\%) &	0.668	 (+2.61	\%) &	0.672	 (+3.23	\%)	\\
% \midrule
% Related Products & Long-click 	&	0.749	 (+2.18	\%) &	0.740	 (+0.95	\%) &	0.738	 (+0.68	\%) &	0.738	 (+0.68	\%) &	0.737	 (+0.55	\%) &	0.741	 (+1.09	\%)	\\
% \midrule
% \multirow{2}{*}{Idea Pin} & Close-ups 	&	0.776	 (+7.18	\%) &	0.749	 (+3.45	\%) &	0.757	 (+4.56	\%) &	0.747	 (+3.18	\%) &	0.746	 (+3.04	\%) &	0.752	 (+3.87	\%)	\\
% & Repin 	&	0.849	 (+6.52	\%) &	0.827	 (+3.76	\%) &	0.833	 (+4.52	\%) &	0.829	 (+4.02	\%) &	0.824	 (+3.39	\%) &	0.827	 (+3.76	\%)	\\
% \midrule
% \multirow{2}{*}{Video} & Close-ups 	&	0.470	 (+5.38	\%) &	0.449	 (+0.67	\%) &	0.454	 (+1.79	\%) &	0.451	 (+1.12	\%) &	0.453	 (+1.57	\%) &	0.451	 (+1.12	\%)	\\
% & Repin 	&	0.603	 (+5.60	\%) &	0.578	 (+1.23	\%) &	0.581	 (+1.75	\%) &	0.575	 (+0.70	\%) &	0.573	 (+0.35	\%) &	0.578	 (+1.23	\%)	\\



% The distributed training of heterogeneous graph models is not straightforward. One needs to develop several modules for supporting distributed training on the heterogeneous graph. These modules should support heterogeneous graph partitioning, neighbor sampling, and GNNs message passing operations. There are a few frameworks such as 
%  This issue of is known data stalling \cite{mohan2020analyzing,kumar2021exploring, kumar2020quiver}.


% Additionally, to the best of our knowledge, the recommendation performance of such frameworks is not known on a billion node heterogeneous graph.  For example, it is uncertain that the proposed graph partitioning strategies will be efficient on a billion scale graph. The second challenge is to address the low model training throughput while training heterogeneous graph models. This is due to latency incurred in sampling the node's neighbors and ingesting the features of sampled neighbors. The problem of low training throughput due to data stalling has been recently studied \cite{mohan2020analyzing,kumar2021exploring, kumar2020quiver}.  require specialized data ingestion pipelines \cite{zhao2021understanding} or efficient cache design \cite{kumar2020quiver, wang2020diesel} to increase the throughput.  These data ingestion designs are proposed for vision/text datasets and cannot be directly extended to graph setup due to specific requirements of random-walker and graph partitioning.

==> problem.tex <==
\xhdr{Notation} Let $q$ be the query item and $e$ an engaged item. Let $x_q$ be the embedding of item $q$ with embedding dimensionality $d$. 
